Neural Graph Reasoning: Complex Logical Query Answering Meets Graph Databases

Complex logical query answering (CLQA) is a recently emerged task of graph machine learning that goes beyond simple one-hop link prediction and solves a far more complex task of multi-hop logical reasoning over massive, potentially incomplete graphs in a latent space. The task received a significant traction in the community; numerous works expanded the field along theoretical and practical axes to tackle different types of complex queries and graph modalities with efficient systems. In this paper, we provide a holistic survey of CLQA with a detailed taxonomy studying the field from multiple angles, including graph types (modality, reasoning domain, background semantics), modeling aspects (encoder, processor, decoder), supported queries (operators, patterns, projected variables), datasets, evaluation metrics, and applications. Refining the CLQA task, we introduce the concept of Neural Graph Databases (NGDBs). Extending the idea of graph databases (graph DBs), NGDB consists of a Neural Graph Storage and a Neural Graph Engine. Inside Neural Graph Storage, we design a graph store, a feature store, and further embed information in a latent embedding store using an encoder. Given a query, Neural Query Engine learns how to perform query planning and execution in order to efficiently retrieve the correct results by interacting with the Neural Graph Storage. Compared with traditional graph DBs, NGDBs allow for a flexible and unified modeling of features in diverse modalities using the embedding store. Moreover, when the graph is incomplete, they can provide robust retrieval of answers which a normal graph DB cannot recover. Finally, we point out promising directions, unsolved problems and applications of NGDB for future research.

==> tables/tab_complexity.tex <==
% \begin{landscape}
\begin{table}[!ht]
\centering
\small
\caption{Time complexity of each operation. \hr{beta/gammae: assume digamma is O(1), perm: weird implementation, all: assume mlp's hidden dim is o(d), assume number of intersection is much much smaller than d, also assume number of intersection/union is constant (otherwise may affect mpqe gnn models), assume the number of qualifiers is a constant (affect starqe), assume the query has $n$ operations}\label{tab:complexity}
\notations{emb-dim = hidden-dim = d; number of projections = r; number of intersection = i; number of union = u; number of layers = l}
}
\resizebox{1.3\columnwidth}{!}{%
\begin{tabular}{ccccccc}
	\toprule
Model & Projection & Intersection & Negation & Union & Answer Retrieval & Comments \\
\hline
GQE / +hashing & \multirow{2}{*}{$\gO(d)$} & \multirow{2}{*}{$\gO((il+1)d^2+id)$} & \multirow{2}{*}{-} & \multirow{2}{*}{-} & \multirow{2}{*}{$\gO(|\gE|d)$} & \\
RotatE/Distmult/ComplEx-m &  &  &  &  & & \\\hline
CGA & $\gO(d^2)$ & $\gO(3kid+d^2)$ & - & - & $\gO(|\gE|d)$ & $k$ is N-attn-head \\\hline
MPQE / GNNQ & \multicolumn{2}{c}{$\gO(d^2n_ql|\gE_q|)$} & - & - & $\gO(|\gE|d)$ & $n_q$ is degree \\\hline
StarQE & \multicolumn{2}{c}{$\gO(d^2n_ql|\gE_q|+|\gS_q||qp|d)$} & - & - & $\gO(|\gE|d)$ & \\\hline
LMPNN & \multicolumn{3}{c}{$\gO(d^2n_ql|\gE_q|)$} & DNF & $\gO(|\gE|d)$ & \\\hline
BiQE & \multicolumn{2}{c}{$\gO((|\gE_q|d^2+|\gE_q|^2d)l)$} & - & - & $\gO(|\gE|d)$\\\hline
kgTransformer & \multicolumn{3}{c}{$\gO(d^2n_ql|\gE_q|+|\gE_q|n_q^2dl)$} & - & $\gO(|\gE|d)$ \\\hline
% Sheaves & & & - & - & \\\hline
Query2Particles & $\gO(Kd^2)$ & $\gO(iKd^2)$ & $\gO(Kd^2)$ & DNF & $\gO(|\gE|dK)$ \\\hline
SignalE & $\gO(d)$ & $\gO(ild^2)$ & $\gO(d)$ & DNF & $\gO(|\gE|d)$ \\\hline
MLPMix & $\gO(d^2l)$ & $\gO(d^2li)$ & $\gO(d^2l)$ & DNF & $\gO(|\gE|d)$ \\\hline
Query2Box / Query2Onto & $\gO(d)$ & $\gO(ild^2)$ & - & DNF & $\gO(|\gE|d)$ \\\hline
RotatE-Box & $\gO(d)$ & - & - & DNF / $\gO(uld^2)$ & $\gO(|\gE|d)$ \\\hline
NewLook & $\gO(|\gE|d+ld^2)$ & $\gO(i(|\gE|+ld^2))$ & $\gO(ld^2)$ & DNF & $\gO(|\gE|d)$ \\\hline
HypE & $\gO(d)$ & $\gO(ild^2)$ & - & DNF & $\gO(|\gE|d)$ \\\hline
ConE/BetaE & $\gO(ld^2)$ & $\gO(ild^2)$ & $\gO(d)$ & DNF & $\gO(|\gE|d)$ \\\hline
PERM & $\gO(d^2)$ & \hr{? require linear solver} & - & \hr{? exp over dist} & \\\hline
LinE & $\gO(ld^2)$ & $\gO(d)$ & $\gO(d)$ & $\gO(d)$ & $\gO(|\gE|d)$ \\\hline
GammaE & $\gO(ld^2)$ & $\gO(ild^2)$ & $\gO(d)$ & $\gO(uld^2)$ & $\gO(|\gE|d)$ \\\hline
NMP-QEM & $\gO(Kld^2)$ & $\gO(iK^2d)$ & $\gO(Kld^2)$ & DNF & $\gO(|\gE|dK)$ \\\hline
EmQL & $\gO(|\gE|d)$ & $\gO(d)$ & - & $\gO(d)$ & $\gO(|\gE|d)$ \\\hline
CQD-CO & $\gO(|\gE|d)$ & Opt & - & Opt & $\gO(|\gE|d)$ \\\hline
CQD-Beam & $\gO(|\gE|d)$ & $k\gO(\gE)d$ & - & $\gO(\gE kd)$ & $\gO(|\gE|d)$ \\\hline
QTO & $\gO(|\gE|\max_k|T^*(v_k)>0|)$ & $\gO(\gE)$ & $\gO(\gE)$ & $\gO(\gE)$ & $\gO(\gE)$ \\\hline
LogicE & $\gO(ld^2)$ & $\gO(d)$ & $\gO(d)$ & $\gO(d)$ & $\gO(|\gE|d)$ \\\hline
FuzzQE & $\gO(d^2)$ & $\gO(d)$ & $\gO(d)$ & $\gO(d)$ & $\gO(|\gE|d)$ \\\hline
TAR & $\gO(d)$ & $\gO(d)$ & $\gO(d)$ & $\gO(d)$ & $\gO(|\gE|d)$ \\\hline
GNN-QE & $\gO(|\gE|d^2+|\gS|d)$ & $\gO(|\gE|)$ & $\gO(|\gE|)$ & $\gO(|\gE|)$ & $\gO(|\gE|)$ \\\hline
FLEX & $\gO(ld^2)$ & $\gO(ild^2)$ & $\gO(ld^2)$ & $\gO(uld^2)$ \hr{super weird} & $\gO(|\gE|d)$ \\\hline
TFLEX & $\gO(ld^2)$ & $\gO(ild^2)$ & $\gO(ld^2)$ & $\gO(uld^2)$ & $\gO(|\gE|d)$ \\\hline
% NQE & & & & & $\gO(|\gE|d)$ \\\hline
\bottomrule
\end{tabular}
}%
\end{table}
% \end{landscape}

==> tables/tab_log.tex <==
% \begin{table}[!ht]

% \begin{subtable}[h]{\textwidth}
% % \centering
% % \caption{Complex Query Answering approaches categorized under \emph{Processor}. \hr{why is newlook symbolic?}\mg{Any Processor - keep or remove?}}
% % \label{tab:processor1}
% % %\scriptsize
% % %\resizebox{\columnwidth}{!}{%
% % \begin{tabular}{cccc}\toprule
% % Any Processor & Neural & Neuro-Symbolic & Symbolic \\
% % \midrule
% % \multicolumn{1}{p{2.5cm}}{TeMP \citeps{temp2022}, NodePiece-QE \citeps{galkin2022}} &
% % \multicolumn{1}{p{8cm}}{GQE \citeps{gqe}, GQE w/ hashing \citeps{gqe_bin}, CGA \citeps{cga}, BiQE \citeps{biqe}, MPQE \citeps{mpqe}, StarQE \citeps{starqe}, MLPMix \citeps{mlpmix},  Query2Particles \citeps{query2particles2022}, KGTrans \citeps{kgtrans2022}, RotatE-m, DistMult-m, ComplEx-m \citeps{smore}, GNNQ \citeps{gnnq}, LMPNN \citeps{lmpnn}} & \multicolumn{1}{p{2cm}}{See below} & \multicolumn{1}{p{3cm}}{TractOR \citeps{tractor2020}, NewLook \citeps{newlook}, CBR-SUBG \citeps{cbr_subg2022}} \\
% % \bottomrule
% % \end{tabular}
% % %}
% \end{subtable}
% %\vfill
% \begin{subtable}[h][\textwidth]
% % % %\resizebox{\columnwidth}{!}{%
% % \begin{tabular}{ccc}\toprule
% % Geometric [Neuro-Symbolic] & Probabilistic [Neuro-Symbolic] & Fuzzy Logic [Neuro-Symbolic] \\
% % \midrule
% % \multicolumn{1}{p{6.5cm}}{Query2Box \citeps{q2b}, Query2Onto \citeps{q2b_onto}, RotatE-Box \citeps{regex}, Knowledge Sheaves \citeps{sheaves}, HypE \citeps{hype}, ConE \citeps{cone}} & \multicolumn{1}{p{4.5cm}}{BetaE \citeps{betae}, PERM \citeps{perm}, LinE \citeps{line2022}, GammaE \citeps{gammae}} & \multicolumn{1}{p{7cm}}{EmQL \citeps{emql}, CQD \citeps{cqd}, LogicE \citeps{logic_e}, FuzzQE \citeps{fuzz_qe}, TAR \citeps{abin_abductive2022}, FLEX \citeps{lin2022flex}, TFLEX \citeps{lin2022tflex}, GNN-QE \citeps{gnn_qe}, ENeSy \citeps{enesy}} \\
% % \bottomrule
% % \end{tabular}
% % %}
% \end{subtable}
% \end{table}



% TADA, fixed the widths
\begin{table}[h]
\label{tab:processors_all}
    \caption{temporary for log}
    \begin{subtable}[h]{\columnwidth}
    \centering
    \caption{Complex Query Answering approaches categorized under the  \emph{Processor} type.}
        %\scriptsize
        \resizebox{\linewidth}{!}{
            \begin{tabular}{cc}
            \toprule
            Query Embeddings & Others \\
            \midrule
            \multicolumn{1}{p{8cm}}{GQE \citeps{gqe}, GQE w/ hashing \citeps{gqe_bin}, CGA \citeps{cga}, Query2Box \citeps{q2b}, BetaE \citeps{betae}, Query2Onto \citeps{q2b_onto}, RotatE-Box \citeps{regex}, ConE \citeps{cone}, PERM \citeps{perm}, NewLook \citeps{newlook}, HypE \citeps{hype}, LogicE \citeps{logic_e}, MLPMix \citeps{mlpmix}, FuzzQE \citeps{fuzz_qe}, LinE \citeps{line2022}, GammaE \citeps{gammae}, Query2Particles \citeps{query2particles2022}, RotatE-m, DistMult-m, ComplEx-m \citeps{smore}} 
            & 
            \multicolumn{1}{p{5cm}}{TractOR \citeps{tractor2020}, MPQE \citeps{mpqe}, EmQL \citeps{emql}, BiQE \citeps{biqe}, CQD \citeps{cqd}, StarQE \citeps{starqe}, GNN-QE \citeps{gnn_qe}, CBR-SUBG \citeps{cbr_subg2022}, KGTrans \citeps{kgtrans2022}, GNNQ \citeps{gnnq}, LMPNN \citeps{lmpnn}} \\
            \bottomrule
            \end{tabular}
        }
        \label{tab:processor1}
    \end{subtable}
\end{table}

==> tables/tab_method.tex <==
% \begin{landscape}
\begin{table}[!ht]
\centering
\caption{Several multi-hop KG embedding models that we consider.\label{tab:kg-model} \hr{add temporal operators for TFLEX?}\hr{add kleen plus for rotate-box?}\mg{rather not, they are the only models with those ops - so let's write them in the text}}
\resizebox{0.95\columnwidth}{!}{%
\begin{tabular}{ccccccc}
	\toprule
Model & Embedding Space & Relation Projection & Intersection & Union & Negation & Distance \\
\hline
GQE & $\Em{q}\in\RR^d$, $\Em{v}\in\RR^d$ & $\Em{q}+\Em{r}$ & $\texttt{DeepSet}(\{\Em{q_i}\})$ & - & - & $\|\Em{q}-\Em{v}\|$ \\\hline
GQE+hashing & $\Em{q}\in \{+1,-1\}^d$, $\Em{v}\in\{+1,-1\}^d$ & $\texttt{sgn}(\Em{q}+\Em{r})$ & $\texttt{sgn}(\texttt{DeepSet}(\{\Em{q_i}\}))$ & - & - & $-\textit{cos}(\Em{q},\Em{v})$ \\\hline
CGA & $\Em{q}\in\RR^d$, $\Em{v}\in\RR^d$ & $\Em{W}_r\Em{q}$ & $\texttt{SelfAttention}(\{\Em{q_i}\})$ & - & - & $-\textit{cos}(\Em{q},\Em{v})$ \\\hline
% TractOR & - & - & - & - & - & - \\\hline
\multirow{2}{*}{Q2B} & \multirow{2}{*}{$\Em{q}\in\RR^{2d}$, $\Em{v}\in\RR^d$} & \multirow{2}{*}{$\Em{q}+\Em{r}$} & $\Ce{q}=\sum_i \mathbf{a}_i\odot\Ce{q_i}$ & \multirow{2}{*}{DNF} & \multirow{2}{*}{-} & \multirow{2}{*}{$\text{dist}_\text{out}+\alpha\text{dist}_\text{in}$}\\
&&&$\Of{q}=\text{min}(\{\Of{q_i}\})\odot\sigma(\texttt{DeepSet}(\{\Of{q_i}\}))$&&\\\hline
% MPQE & - & - & - & - & - & - \\\hline
\multirow{2}{*}{RotatE-Box} & \multirow{2}{*}{$\Em{q}\in\CC^{2d},\Em{v}\in\CC^d$} & \multirow{2}{*}{$(\Ce{q}\circ \Ce{r},\Of{q}+\Of{r})$} & \multirow{2}{*}{-} & DNF /  & \multirow{2}{*}{-} & \multirow{2}{*}{$\text{dist}_\text{out}+\alpha\text{dist}_\text{in}$} \\
&&&&$\texttt{DeepSet}(\{\Em{q}_i\})$&\\\hline
% BiQE & - & - & - & - & - & - \\\hline % Non-query embedding
% kgTransformer & - & - & - & - & - & - \\\hline
EmQL & - & - & - & - & - & - \\\hline
Sheave & - & - & - & - & - & - \\\hline
% CQD & - & - & - & - & - & - \\\hline
% HypE & - & - & - & - & - & - \\\hline
NewLook & - & - & - & - & - & - \\\hline
% CBR-SUBG & - & - & - & - & - & - \\\hline
BetaE & $\Em{q}\in\RR^{2d}$, $\Em{v}\in\RR^{2d}$ & $\texttt{MLP}(\Em{q},\Em{r})$ & $\Em{q}=[(\sum w_i\alpha_i,\sum w_i \beta_i)]$ & DNF/DM & $\frac{1}{\Em{q}}$ & $\texttt{KL}(\Em{v};\Em{q})$\\\hline
\multirow{2}{*}{ConE} & $\Em{q}=(\vtheta_\text{ax}, \vtheta_\text{ap})$, $\Em{v}=(\vtheta_\text{ax},\vzero)$ & $g(\texttt{MLP}(\Em{q}+\Em{r}))$ & $\vtheta_\text{ax}=\texttt{SemanticAverage}(\Em{q}_1, \dots, \Em{q}_n)$ & \multirow{2}{*}{DNF/DM} & $\vtheta_\text{ax}=\vone[\vtheta_\text{ax}\geq\vzero](\vtheta_\text{ax}-\pi)$ & \multirow{2}{*}{$\text{dist}_\text{o}+\lambda \text{dist}_\text{i}$} \\&$\vtheta_\text{ax}\in[-\pi,\pi)^d, \vtheta_\text{ap}\in[0,2\pi]^d$ & $g$ generates valid $\vtheta_\text{ax}$ and $\vtheta_\text{ap}$ &$\vtheta_\text{ap}=\texttt{CardMin}(\Em{q}_1, \dots, \Em{q}_n)$& &  $+\vone[\vtheta_\text{ax}<\vzero](\vtheta_\text{ax}+\pi)$, $\vtheta_\text{ap}=2\pi - \vtheta_\text{ap}$ & \\\hline
\multirow{2}{*}{PERM} & \multirow{2}{*}{$\Em{q},\Em{v}=\gN(\vmu,\Sigma)$} & \multirow{2}{*}{$\gN(\vmu_q+\vmu_r, (\Sigma_q^{-1}+\Sigma_r^{-1})^{-1})$} & $\Sigma_q^{-1}=\Sigma_{q_1}^{-1}+\Sigma_{q_2}^{-1}$ & \multirow{2}{*}{$\sum_{i=1} \mathbf{a}_i \gN(\vmu_{q_i}, \Sigma_{q_i})$} & \multirow{2}{*}{-} &  \multirow{2}{*}{$(\vmu_q-\vmu_v)^T\Sigma_q^{-1}(\vmu_q-\vmu_v)$} \\
 & & & $\vmu_q=\Sigma_q(\Sigma_{q_2}^{-1}\vmu_1 + \Sigma_{q_1}^{-1}\vmu_2)$ & & & \\\hline
LogicE & $\Em{q},\Em{v}=([l_i,u_i]\: : \: l_i, u_i \in [0,1])_{i=1}^d$ & $\sigma(\max(0,\max(0,[\Em{r},\Em{q}]\rmF_1)\rmF_2)\rmF_3)$ & $([\top(l_i^{(1)}, \dots, l_i^{(n)}),\top(u_i^{(1)}, \dots, u_i^{(n)})])_{i=1}^d$ & DM & $([1-l_i, 1-u_i])_{i=1}^d$ & $\sum_{i=1}^d \frac{\|l_i^q - l_i^v\|+\|u_i^q - u_i^v\|}{2d}$ \\\hline
MLPMix & $\Em{q}\in\RR^d$, $\Em{v}\in\RR^d$ & $\texttt{MLP}_\texttt{mix}(\Em{q}, \Em{r})$ & $\texttt{MLP}_\texttt{mix}(\Em{q_1}, \Em{q_2})$ & DNF & $\texttt{MLP}(\Em{q})$ & $\|\Em{q} - \Em{v}\|$ \\\hline
MPQE & $\Em{q}\in\RR^d$, $\Em{v}\in\RR^d$ & $\Em{W}_r\Em{q}$ & $\texttt{RGCN}(\Em{q}, \gG_q)$ & - & - & $\textit{cos}(\Em{q}, \Em{v})$ \\\hline
StarQE & $\Em{q}\in\RR^d$, $\Em{v}\in\RR^d$ & $f(\Em{q}, g(\Em{r}, \Em{h}_{\text{qualifiers}}))$ & $\texttt{GNN}(\Em{q}, \gG_q)$ & - & - & $\texttt{dot}(\Em{q},\Em{v})$ \\\hline
\multirow{2}{*}{FuzzQE} & \multirow{2}{*}{$\Em{q}\in[0,1]^d, \Em{v}\in[0,1]^d$} & $g(\texttt{MLP}(\Em{q}, \Em{r}))$ & Product Logic: $\Em{q_1}\cdot\Em{q_2}$ & $\Em{q_1}+\Em{q_2}-\Em{q_1}\cdot\Em{q_2}$ & $\Em{1}-\Em{q}$ & \multirow{2}{*}{$-\texttt{L2Norm}(\phi(\Em{q}, \Em{v}))$} \\
&&$g$ constrains the output to $[0,1]^d$&G\"odex Logic: $\text{min}(\Em{q_1}, \Em{q_2})$ &$\text{max}(\Em{q_1}, \Em{q_2})$& - & \\\hline
GNN-QE &  $\Em{q}\in\RR^d$ & $\sigma(\texttt{GNN}(\Em{q},\gG))$ &  $\Em{q_1}\cdot\Em{q_2}$ & $\Em{q_1}+\Em{q_2}-\Em{q_1}\cdot\Em{q_2}$ & $\Em{1}-\Em{q}$ & $\texttt{BCE}(\Em{q})$ \\\hline
% GNNQ & - & - & - & - & - & - \\\hline
ENeSy & - & - & - & - & - & - \\\hline
LMPNN & - & - & - & - & - & - \\\hline
LinE & $\Em{q},\Em{v}=[(p_{j,1},\dots,p_{j,k})]_{j=1}^h\in\RR^{k\times h}$ & $\texttt{MLP}(\Em{q}, \Em{r})$ & $[\text{min}(p_1^{q_1},\dots,p_1^{q_n}),\dots,\text{min}(p_k^{q_1},\dots,p_k^{q_n})]^h$ & $[\text{max}(p_1^{q_1},\dots,p_1^{q_n}),\dots,\text{max}(p_k^{q_1},\dots,p_k^{q_n})]^h$ & $[\frac{1}{p_1^q},\dots,\frac{1}{p_k^q}]^h$ & $\|\Em{q} - \Em{v}\|^2_2$ \\\hline
\multirow{2}{*}{Query2Particles} & \multirow{2}{*}{$\Em{q},\Em{v}=[p^1, \dots, p^K]\in\RR^{d\times K}$} & $f(\Em{q}, \Em{r})$ & $\Em{q_I}=[\Em{q}^1, \dots, \Em{q}^N]\in\RR^{d\times NK}$ & \multirow{2}{*}{$[\Em{q}^1, \dots, \Em{q}^N]$} & $\Em{q_C}=[\Em{q}^1, \dots, \Em{q}^N]\in\RR^{d\times NK}$ & \multirow{2}{*}{$-\max_{k\in\{1,\dots,K\}} <\Em{q}^k, \Em{v}> $} \\
&&$f$ is neuralized gates. &$\texttt{MLP}(\texttt{Attn}(W_q^I \Em{q_I}^T,W_k^I \Em{q_I}^T,W_v^I \Em{q_I}^T)^T)$&&$\texttt{MLP}(\texttt{Attn}(W_q^C \Em{q_C}^T,W_k^C \Em{q_C}^T,W_v^C \Em{q_C}^T)^T)$&\\\hline
TAR & $\Em{q}\in\RR^d, \Em{v}\in\RR^d$ & $\Em{q}+\Em{r}$ & $\sum_{i=1}^{2} \texttt{Attn}(\texttt{MLP}(\Em{q}_1 \oplus \Em{q}_2 )) *\Em{q}_i$ & $\textit{max}(\Em{q}_1, \Em{q}_2)$ & $1-\Em{q}$ & $\|\Em{q}-\Em{v}\|$ \\\hline
% TEMP & - & - & - & - & - & - \\\hline
\multirow{2}{*}{FLEX} & $\Em{q}=(\Em{\theta}_f, \Em{\theta}_l), \Em{\theta}_f\in[-L,L]^d, \Em{\theta}_l\in[0,1]^d$ & $g(\texttt{MLP}([\Em{\theta}_f + \Em{\theta}_{f,r};\Em{\theta}_l + \Em{\theta}_{l,r}]))$ & $\Em{\theta}_f=\sum_i \mathbf{a}_i\Em{\theta}_{q_i,f}$ & $\Em{\theta}_f=\sum_i \mathbf{a}_i\Em{\theta}_{q_i,f}$ & $L \text{tanh}(\texttt{MLP}([\Em{\theta}_f;\Em{\theta}_l]))$ & \multirow{2}{*}{$\|\Em{\theta}_{v,f} - \Em{\theta}_{q,f}\|_1 + \Em{\theta}_{q,l}$} \\
& $\Em{v}=(\Em{\theta}_f,\Em{0}), \Em{\theta}_f\in[-L,L]^d$ & $g$ generates valid $\Em{\theta}_f$ and $\Em{\theta}_v$. & $\Em{\theta}_l=\Pi_i \Em{\theta}_{q_i,l}$ & $\Em{\theta}_l=\sum_i \Em{\theta}_{q_i,l} - \sum_{1\leq i<j\leq n}\Em{\theta}_{q_i,l}\Em{\theta}_{q_j,l} + \dots + (-1)^{n-1}\Pi_i \Em{\theta}_{q_i,l}$ & $1 - \Em{\theta}_l $& \\\hline
\multirow{2}{*}{TFLEX} & $\Em{q}=(\Em{q}_f^e,\Em{q}_l^e,\Em{q}_f^t,\Em{q}_l^t), \Em{q}_f^e,\Em{q}_f^t\in\RR^d,\Em{q}_l^e,\Em{q}_l^t\in[0,1]^d$ & $\gP_e(\Em{q},\Em{r},\Em{t})=g(\texttt{MLP}([\Em{q} + \Em{r} + \Em{t}))$ & $\gI_e(\Em{q_1},\dots,\Em{q_n}) = (\sum_i \mathbf{\alpha}\Em{q}_{i,f}^e, \textbf{AND}_i(\{\Em{q}_{i,l}^e\}), \sum_i \mathbf{\beta}\Em{q}_{i,f}^t, \textbf{AND}_i(\{\Em{q}_{i,l}^t\}))$ & $\gU_e(\Em{q_1},\dots,\Em{q_n}) = (\sum_i \mathbf{\alpha}\Em{q}_{i,f}^e, \textbf{OR}_i(\{\Em{q}_{i,l}^e\}), \sum_i \mathbf{\beta}\Em{q}_{i,f}^t, \textbf{AND}_i(\{\Em{q}_{i,l}^t\}))$ & $\gC_e(\Em{q})=(f_\text{not}^e(\Em{q}_f^e),\textbf{NOT}(\Em{q}_l^e),\Em{q}_f^t, \Em{q}_l^t)$ & $d^e(\Em{v};\Em{q})=\|\Em{v}_f^e - \Em{q}_f^e\|_1+\Em{q}_l^e$ \\
& $\Em{v}=(\Em{v}_f^e,\Em{0},\Em{0},\Em{0}), \Em{v}_f^e\in\RR^d$ & $\gP_t(\Em{q_1},\Em{r},\Em{q_2})=g(\texttt{MLP}([\Em{q} + \Em{r} + \Em{q_2}))$ & $\gI_t(\Em{q_1},\dots,\Em{q_n}) = (\sum_i \mathbf{\alpha}\Em{q}_{i,f}^e, \textbf{AND}_i(\{\Em{q}_{i,l}^e\}), \sum_i \mathbf{\beta}\Em{q}_{i,f}^t, \textbf{AND}_i(\{\Em{q}_{i,l}^t\}))$ & $\gU_t(\Em{q_1},\dots,\Em{q_n}) = (\sum_i \mathbf{\alpha}\Em{q}_{i,f}^e, \textbf{OR}_i(\{\Em{q}_{i,l}^e\}), \sum_i \mathbf{\beta}\Em{q}_{i,f}^t, \textbf{AND}_i(\{\Em{q}_{i,l}^t\}))$ & $\gC_t(\Em{q})=(\Em{q}_f^e, \Em{q}_l^e,f_\text{not}^t(\Em{q}_f^t),\textbf{NOT}(\Em{q}_l^t))$ & $d^t(\Em{t};\Em{q})=\|\Em{t}_f^t - \Em{q}_f^t\|_1+\Em{q}_l^t$ \\\hline
RotatE-m & $\Em{q}\in\CC^{d}$,$\Em{v}\in\CC^{d}$ & $\Em{q}\circ\Em{r}$ & $\texttt{DeepSet}(\{\Em{q_i}\})$ & - & - & $\|\Em{q}-\Em{r}\|$ \\\hline
DisMult-m & $\Em{q}\in\RR^d$, $\Em{v}\in\RR^d$ & $\texttt{L2Norm}(\Em{q}\circ\Em{r})$ & $\texttt{L2Norm}(\texttt{DeepSet}(\{\Em{q_i}\}))$ & - & - & $-<\Em{q},\Em{v}>$ \\\hline
ComplEx-m & $\Em{q}\in\CC^{d}$, $\Em{v}\in\CC^{d}$ & $\texttt{L2Norm}(\Em{q}\circ\Em{r})$ & $\texttt{L2Norm}(\texttt{DeepSet}(\{\Em{q_i}\}))$ & - & - & $-\text{Re}(<\Em{q},\overline{\Em{v}}>)$ \\
	\bottomrule
\end{tabular}
}%
\end{table}
% \end{landscape}

==> tikz/taxonomy_big.tex <==
\forestset{
%   tracks/.style={
%     for tree={
%       grow'=0,
%       l sep'+=50pt,
%       s sep'+=30pt,
%       font=\bfseries\sffamily,
%       edge path'={
%         (!u.parent anchor) -- ($(.child anchor)-(20pt,0pt)$) -- (.child anchor)
%       },
%       edge+={ultra thick, rounded corners}
%     },
%     before typesetting nodes={
%       for descendants={
%         edge label/.process={ Ow {content} {node [above, font=\bfseries\sffamily, anchor=south, pos=.75] {##1}} },
%         content=,
%         shape=coordinate,
%       },
%       where={>Ow+P {n children} {isodd(##1)} }{
%         calign=child edge,
%         calign primary child/.process={ Ow+n {n children} {(##1+1)/2} }
%       }{}  
%     },
%   },
  L1/.style={rectangle, draw, fill=blue!20!red!20, rounded corners, thick,edge={line width=0.5pt}},
  L2/.style={rectangle, draw, fill=blue!20!green!20, rounded corners, thick,edge={line width=0.5pt}},
  L25/.style={rectangle, draw, fill=blue!20!green!20, rounded corners, thick,edge={line width=0.5pt}, text width=3cm},
  L3/.style={rectangle, draw, fill=gray!20, rounded corners, thick,edge={line width=0.5pt}, text width=3cm},
  L4/.style={rectangle, draw, fill=blue!15, rounded corners, thick,edge={line width=0.5pt}},
  L45/.style={rectangle, draw, fill=blue!15, rounded corners, thick,edge={line width=0.5pt}, text width=3cm},
  L5/.style={rectangle, draw, fill=yellow!20, rounded corners, thick,edge={line width=0.5pt}},
  L55/.style={rectangle, draw, fill=yellow!20, rounded corners, thick,edge={line width=0.5pt}, text width=3cm},
  %%%%%%%%%%%%%
}
%\hspace{2in}
%\\
\begin{forest}
    %forked edges,
    for tree={
        % %align=center, % allow multiple lines
        % grow=0,
        % draw,
        % reversed, % tree direction
        % parent anchor=east,child anchor=west, % edge anchors
        % edge path'={
        % (!u.parent anchor) -- ($(.child anchor)-(10pt,0pt)$) -- (.child anchor)
        % },
        % edge={line cap=round,rounded corners},
        % outer sep=+1.5pt, % edge/node connection
        % rounded corners,
        % minimum width=15mm,
        % minimum height=8mm, % node shape
        % %l sep=15mm, % level distance
        % s sep=6pt,
        % calign=edge midpoint,
        % node options={align=center,},
        forked edges,
        grow'=0,
        draw,
        rounded corners,
        node options={align=center,},
        text width=19cm,
        s sep=6pt,
        calign=edge midpoint,
    }
    [\textbf{Neural} \\
    \textbf{Query Engine},L3
        [\textbf{Graph}\\{\hyperref[sec:graphs]{Section \ref{sec:graphs}}},L3
            [Modality,L3
                [Triple KGs,L55
                    % [{GQE\cite{gqe, gqe_bin}, Query2Box\cite{q2b}, BetaE\cite{betae}, EmQL\cite{emql}, MPQE\cite{mpqe}, BiQE\cite{biqe} \\,  \cite{sheaves}, HypE\cite{hype}, NewLook\cite{newlook}, CQD\cite{cqd}, PERM\cite{perm}, ConE\cite{cone}},L5
                    % ]
                    [\citet{gqe, gqe_bin, q2b, betae, emql, sheaves, mpqe, biqe, hype, newlook, cqd, perm, cone, q2b_onto, logic_e, mlpmix, fuzz_qe, gnn_qe, cbr_subg2022, smore, kgtrans2022, line2022, query2particles2022, abin_abductive2022, temp2022, lin2022flex, lin2022tflex}, L5]
                ]
                [Hyper-Relational KGs,L55
                    [ StarQE \citet{starqe} ,L5
                    ]
                ]
                [Hypergraphs,L55
                    [None,L55
                    ]
                ]
                [Multi-modal KGs,L55
                    [None ,L55
                    ]
                ]
            ]
            [Reasoning Domain,L3
                [Discrete,L55
                    [\citet{gqe, gqe_bin, q2b, betae, emql, sheaves, mpqe, biqe, hype, newlook, cqd, perm, cone, q2b_onto, logic_e, mlpmix, fuzz_qe, gnn_qe, cbr_subg2022, smore, kgtrans2022, line2022, query2particles2022, abin_abductive2022, temp2022, lin2022flex, starqe}, L5]
                ]
                [Discrete + Time,L55
                    [TFLEX \citet{lin2022tflex},L5
                    ]
                ]
                [Discrete + Continuous,L55
                    [None,L55
                    ]
                ]
            ]   
            [Expressiveness,L3
                [EPFO,L55
                    [\citet{gqe, gqe_bin, q2b, emql, sheaves, mpqe, biqe, hype, newlook, cqd, q2b_onto, cbr_subg2022, kgtrans2022, starqe}, L5]
                ]
                [EPFO + Negation,L55
                    [\citet{betae, cone, perm, logic_e, mlpmix, gnn_qe, fuzz_qe, line2022, query2particles2022, lin2022flex, lin2022tflex}, L5]
                ]
                [Class Hierarchies \\ (TBOX),L55
                    [\citet{q2b_onto, temp2022, abin_abductive2022}, L5]
                ]
                [OWL Profiles,L55
                    [None,L55
                    ]
                ]
            ]
        ]
        [\textbf{Learning}\\ {\hyperref[sec:learning]{Section \ref{sec:learning}}},L3
            [Learning,L3
                [Transductive,L25
                    [\citet{gqe, gqe_bin, q2b, betae, emql, sheaves, mpqe, biqe, hype, newlook, perm, cone, q2b_onto, logic_e, mlpmix, fuzz_qe, cbr_subg2022, smore, kgtrans2022, line2022, query2particles2022, abin_abductive2022, lin2022flex, lin2022tflex, starqe}, L2]
                ]
                [Inductive \\ (limited),L25
                    [Temp \citet{temp2022},L2
                    ]
                ]
                [Inductive,L25
                    [{GNN-QE\citet{gnn_qe}, CQD\citet{cqd}},L2
                    ]
                ]
            ]
            [Modeling,L3
                [Neural,L25
                    [\citet{gqe, gqe_bin, biqe, mlpmix,  kgtrans2022,  temp2022}, L2]
                ]
                [Neuro-Symbolic,L25
                    [GNN-based, L25
                        [\citet{mpqe, starqe, gnn_qe}, L2]
                    ]
                    [Geometric, L25
                        [\citet{q2b, q2b_onto, sheaves,  hype, cone,  query2particles2022}, L2]
                    ]
                    [Probabilistic, L25
                        [\citet{betae, perm, line2022}, L2]
                    ]
                    [Fuzzy Logic, L25
                        [\citet{emql, cqd, logic_e, fuzz_qe, abin_abductive2022, lin2022flex, lin2022tflex}, L2]
                    ]
                ]
                [Symbolic,L25
                    [\citet{newlook, cbr_subg2022}, L2]
                ]
            ]
            [Training,L3
                [End-to-end,L25
                    [\citet{gqe, gqe_bin, q2b, betae, emql, sheaves, mpqe, biqe, hype, newlook, perm, cone, q2b_onto, logic_e, mlpmix, fuzz_qe, gnn_qe, cbr_subg2022, smore, kgtrans2022, line2022, query2particles2022, abin_abductive2022, temp2022, lin2022flex, lin2022tflex, starqe}, L2]
                ]
                [Inference-only,L25
                    [CQD \citet{cqd},L2
                    ]
                ]
            ]
        ]
        [\textbf{Queries}\\ {\hyperref[sec:queries]{Section \ref{sec:queries}}},L3
            [Query Operators,L3
                [Projection + JOIN,L45
                    [\citet{gqe, gqe_bin, mpqe, sheaves, biqe, starqe, cbr_subg2022},L4
                    ]
                ]
                [+ UNION,L45
                    [\citet{q2b, emql, q2b_onto, hype, newlook, cqd, kgtrans2022, abin_abductive2022},L4
                    ]
                ]
                [+ NOT,L45
                    [\citet{betae, cone, perm, logic_e, mlpmix, fuzz_qe, gnn_qe, smore, line2022, query2particles2022, temp2022, lin2022flex, lin2022tflex},L4
                    ]
                ]
                [Filter,L45
                    [None,L45
                    ]
                ]
                [Aggregations,L45
                    [None,L45
                    ]
                ]
            ]
            [Query Patterns,L3
                [Fixed set,L45
                    [\textbf{TODO},L45
                    ]
                ]
                [Arbitrary DAGs,L45
                    [TODO;  \citet{biqe},L4
                    ]
                ]
                [Extended DAGs,L45
                    [TODO; \citet{starqe, lin2022tflex},L4
                    ]
                ]
                [Cyclic patterns,L45
                    [None,L45]
                ]
            ]
            [Projected Variables,L3
                [Final nodes only,L45
                    [\citet{gqe, gqe_bin, mpqe, sheaves, mlpmix, starqe, cbr_subg2022} ,L4
                    ]
                ]
                [Arbitrary \\ non-anchor nodes,L45
                    [\citet{q2b, betae, emql, biqe, cqd, hype, newlook, cone, perm, q2b_onto, logic_e, fuzz_qe, gnn_qe, smore, kgtrans2022, line2022, query2particles2022, abin_abductive2022, temp2022, lin2022flex, lin2022tflex} ,L4
                    ]
                ]
                [Arbitrary non-anchor \\ nodes + literals,L45
                    [None ,L45
                    ]
                ]
            ]
        ]
    ]   
\end{forest}
%}
%} 

==> tikz/taxonomy_small.tex <==
\forestset{
%   tracks/.style={
%     for tree={
%       grow'=0,
%       l sep'+=50pt,
%       s sep'+=30pt,
%       font=\bfseries\sffamily,
%       edge path'={
%         (!u.parent anchor) -- ($(.child anchor)-(20pt,0pt)$) -- (.child anchor)
%       },
%       edge+={ultra thick, rounded corners}
%     },
%     before typesetting nodes={
%       for descendants={
%         edge label/.process={ Ow {content} {node [above, font=\bfseries\sffamily, anchor=south, pos=.75] {##1}} },
%         content=,
%         shape=coordinate,
%       },
%       where={>Ow+P {n children} {isodd(##1)} }{
%         calign=child edge,
%         calign primary child/.process={ Ow+n {n children} {(##1+1)/2} }
%       }{}  
%     },
%   },
  L1/.style={rectangle, draw, fill=blue!20!red!20, rounded corners, thick,edge={line width=0.5pt}},
  L2/.style={rectangle, draw, fill=blue!20!green!20, rounded corners, thick,edge={line width=0.5pt}},
  L25/.style={rectangle, draw, fill=blue!20!green!20, rounded corners, thick,edge={line width=0.5pt}, text width=3cm},
  L3/.style={rectangle, draw, fill=gray!20, rounded corners, thick,edge={line width=0.5pt}, text width=3.5cm},
  L4/.style={rectangle, draw, fill=blue!15, rounded corners, thick,edge={line width=0.5pt}},
  L45/.style={rectangle, draw, fill=blue!15, rounded corners, thick,edge={line width=0.5pt}, text width=3cm},
  L5/.style={rectangle, draw, fill=yellow!20, rounded corners, thick,edge={line width=0.5pt}},
  L55/.style={rectangle, draw, fill=yellow!20, rounded corners, thick,edge={line width=0.5pt}, text width=3cm},
  %%%%%%%%%%%%%
}
%\hspace{2in}
%\\
\begin{forest}
    %forked edges,
    for tree={
        % %align=center, % allow multiple lines
        % grow=0,
        % draw,
        % reversed, % tree direction
        % parent anchor=east,child anchor=west, % edge anchors
        % edge path'={
        % (!u.parent anchor) -- ($(.child anchor)-(10pt,0pt)$) -- (.child anchor)
        % },
        % edge={line cap=round,rounded corners},
        % outer sep=+1.5pt, % edge/node connection
        % rounded corners,
        % minimum width=15mm,
        % minimum height=8mm, % node shape
        % %l sep=15mm, % level distance
        % s sep=6pt,
        % calign=edge midpoint,
        % node options={align=center,},
        forked edges,
        grow'=0,
        draw,
        rounded corners,
        node options={align=left,},
        text width=5cm,
        s sep=6pt,
        calign=edge midpoint,
    }
    [\textbf{Neural} \\
    \textbf{Query Engine},L3
        [\textbf{Graph},L3
            [Modality,L3
                [Triple KGs,L5
                    % [{GQE\cite{gqe, gqe_bin}, Query2Box\cite{q2b}, BetaE\cite{betae}, EmQL\cite{emql}, MPQE\cite{mpqe}, BiQE\cite{biqe} \\,  \cite{sheaves}, HypE\cite{hype}, NewLook\cite{newlook}, CQD\cite{cqd}, PERM\cite{perm}, ConE\cite{cone}},L5
                    % ]
                    % [\citet{gqe, gqe_bin, q2b, betae, emql, sheaves, mpqe, biqe, hype, newlook, cqd, perm, cone, q2b_onto, logic_e, mlpmix, fuzz_qe, gnn_qe, cbr_subg2022, smore, kgtrans2022, line2022, query2particles2022, abin_abductive2022, temp2022, lin2022flex, lin2022tflex}, L5]
                ]
                [Hyper-Relational KGs,L5
                    % [ StarQE \citet{starqe} ,L5
                    % ]
                ]
                [Hypergraphs,L5
                    % [None,L55
                    % ]
                ]
                [Multi-modal KGs,L5
                    % [None ,L55
                    % ]
                ]
            ]
            [Reasoning Domain,L3
                [Discrete,L5
                    % [\citet{gqe, gqe_bin, q2b, betae, emql, sheaves, mpqe, biqe, hype, newlook, cqd, perm, cone, q2b_onto, logic_e, mlpmix, fuzz_qe, gnn_qe, cbr_subg2022, smore, kgtrans2022, line2022, query2particles2022, abin_abductive2022, temp2022, lin2022flex, starqe}, L5]
                ]
                [Discrete + Time,L5
                    % [TFLEX \citet{lin2022tflex},L5
                    % ]
                ]
                [Discrete + Continuous,L5
                    % [None,L55
                    % ]
                ]
            ]   
            [Expressiveness,L3
                [EPFO,L5
                    % [\citet{gqe, gqe_bin, q2b, emql, sheaves, mpqe, biqe, hype, newlook, cqd, q2b_onto, cbr_subg2022, kgtrans2022, starqe}, L5]
                ]
                [EPFO + Negation,L5
                    % [\citet{betae, cone, perm, logic_e, mlpmix, gnn_qe, fuzz_qe, line2022, query2particles2022, lin2022flex, lin2022tflex}, L5]
                ]
                [Class Hierarchies (TBOX),L5
                    % [\citet{q2b_onto, temp2022, abin_abductive2022}, L5]
                ]
                [OWL Profiles,L5
                    % [None,L55
                    % ]
                ]
            ]
        ]
        [\textbf{Learning},L3
            [Learning,L3
                [Transductive,L2
                    % [\citet{gqe, gqe_bin, q2b, betae, emql, sheaves, mpqe, biqe, hype, newlook, perm, cone, q2b_onto, logic_e, mlpmix, fuzz_qe, cbr_subg2022, smore, kgtrans2022, line2022, query2particles2022, abin_abductive2022, lin2022flex, lin2022tflex, starqe}, L2]
                ]
                [Inductive (limited),L2
                    % [Temp \citet{temp2022},L2
                    % ]
                ]
                [Inductive,L2
                    % [{GNN-QE\citet{gnn_qe}, CQD\citet{cqd}},L2
                    % ]
                ]
            ]
            [Modeling,L3
                [Neural,L25
                    % [\citet{gqe, gqe_bin, biqe, mlpmix,  kgtrans2022,  temp2022}, L2]
                ]
                [Neuro-Symbolic,L25
                    [GNN-based, L25
                        % [\citet{mpqe, starqe, gnn_qe}, L2]
                    ]
                    [Geometric, L25
                        % [\citet{q2b, q2b_onto, sheaves,  hype, cone,  query2particles2022}, L2]
                    ]
                    [Probabilistic, L25
                        % [\citet{betae, perm, line2022}, L2]
                    ]
                    [Fuzzy Logic, L25
                        % [\citet{emql, cqd, logic_e, fuzz_qe, abin_abductive2022, lin2022flex, lin2022tflex}, L2]
                    ]
                ]
                [Symbolic,L25
                    % [\citet{newlook, cbr_subg2022}, L2]
                ]
            ]
            [Training,L3
                [End-to-end,L25
                    % [\citet{gqe, gqe_bin, q2b, betae, emql, sheaves, mpqe, biqe, hype, newlook, perm, cone, q2b_onto, logic_e, mlpmix, fuzz_qe, gnn_qe, cbr_subg2022, smore, kgtrans2022, line2022, query2particles2022, abin_abductive2022, temp2022, lin2022flex, lin2022tflex, starqe}, L2]
                ]
                [Inference-only,L25
                    % [CQD \citet{cqd},L2
                    % ]
                ]
            ]
        ]
        [\textbf{Queries},L3
            [Query Operators,L3
                [Projection + JOIN,L4
                    % [\citet{gqe, gqe_bin, mpqe, sheaves, biqe, starqe, cbr_subg2022},L4
                    % ]
                ]
                [+ UNION,L4
                    % [\citet{q2b, emql, q2b_onto, hype, newlook, cqd, kgtrans2022, abin_abductive2022},L4
                    % ]
                ]
                [+ NOT,L4
                    % [\citet{betae, cone, perm, logic_e, mlpmix, fuzz_qe, gnn_qe, smore, line2022, query2particles2022, temp2022, lin2022flex, lin2022tflex},L4
                    % ]
                ]
                [Filter,L4
                    % [None,L45
                    % ]
                ]
                [Aggregations,L4
                    % [None,L45
                    % ]
                ]
            ]
            [Query Patterns,L3
                [Fixed set,L4
                    % [\textbf{TODO},L45
                    % ]
                ]
                [Arbitrary DAGs,L4
                    % [TODO;  \citet{biqe},L4
                    % ]
                ]
                [Extended DAGs,L4
                    % [TODO; \citet{starqe, lin2022tflex},L4
                    % ]
                ]
                [Cyclic patterns,L4
                    % [None,L45]
                ]
            ]
            [Projected Variables,L3
                [Final nodes only,L4
                    % [\citet{gqe, gqe_bin, mpqe, sheaves, mlpmix, starqe, cbr_subg2022} ,L4
                    % ]
                ]
                [Arbitrary non-anchor nodes,L4
                    % [\citet{q2b, betae, emql, biqe, cqd, hype, newlook, cone, perm, q2b_onto, logic_e, fuzz_qe, gnn_qe, smore, kgtrans2022, line2022, query2particles2022, abin_abductive2022, temp2022, lin2022flex, lin2022tflex} ,L4
                    % ]
                ]
                [Arbitrary non-anchor nodes + literals,L4
                    % [None ,L45
                    % ]
                ]
            ]
        ]
    ]   
\end{forest}
%}
%} 
